Developing a Correlation Indices to Identify Coordinated Cyber-Attacks on Power Grids

Increasing reliance on Information and Communication Technology~(ICT) exposes the power grid to cyber-attacks. In particular, Coordinated Cyber-Attacks (CCAs) are considered highly threatening and difficult to defend against, because they (i) possess higher disruptiveness by integrating greater resources from multiple attack entities, and (ii) present heterogeneous traits in cyber-space and the physical grid by hitting multiple targets to achieve the attack goal. Thus, and as opposed to independent attacks, whose severity is limited by the power grid's redundancy, CCAs could inflict disastrous consequences, such as blackouts. In this paper, we propose a method to develop Correlation Indices to defend against CCAs on static control applications. These proposed indices relate the targets of CCAs with attack goals on the power grid. Compared to related works, the proposed indices present the benefits of deployment simplicity and are capable of detecting more sophisticated attacks, such as measurement attacks. We demonstrate our method using measurement attacks against Security Constrained Economic Dispatch.

==> MultipleGoals.tex <==
\subsection{CIs for Multiple Attack Goals.} 
Extending our approach to multiple attack goals is important because it allows us to study the attack's final consequences (\eg cascading blackouts might occur if the adversary congests a set of target lines). 

We can achieve this by adapting the attack template used to derive CIs for a single goal in order to study CCAs with multiple goals. This, however, greatly increases the number of computations. This is because, for a given congestion~($\tilde{\tau}$), if we consider CCAs against individual lines, then we have to compute $m$ collections of CIs. But if we consider CCAs against multiple lines, then we have to compute $2^m$ collections of CIs, which could be computationally prohibitive for large scale power grids (even though we compute CIs offline). Thus, we propose computing CIs for multiple goals using set operations and the CIs for single goals, which we describe in the following proposition and remark.

\textit{Notation:} We model CCAs against multiple goals as follows. Let $J \subset \{1,\hdots,m\}$ be an index set; then we denote the CCA that reaches multiple goals as $\Sa \to \bigwedge_{j \in J} (e_j,\tilde{\tau}_j)$. We use the \textit{and} operator ``$\bigwedge$'' to emphasize that the adversary congests~$(\tilde{\tau}_j)$ (simultaneously) the set of transmission lines $\{e_j \in E~|~j \in J \}$.
\begin{proposition} \label{prop:3}
Let $J$ be an index set, and let $\Sp \in \mathcal{S}^*_{\alpha}(\bigwedge_{j \in J}(e_j,\tilde{\tau}_j))$ be a (not necessarily unique) CI, \ie $\Sp \to \bigwedge_{j \in J}(e_j,\tilde{\tau}_j)$. Moreover, for all $j \in J$, let $\CI \in \mathcal{S}_\alpha^*(e_j,\tilde{\tau}_j)$ be a CI that reaches the single goal $(e_j,\tilde{\tau}_j)$. Then, $\Sp$ satisfies \[|\Sp| \geq \max \{|\CI|~|~j \in J \}.\] 
\end{proposition}
\begin{proof}
Appendix.
\end{proof}

\begin{remark} \label{remark:Multiple}
In fact, under the same assumptions of Proposition~\ref{prop:3}, the CI for multiple goals includes (except in a few cases) the individual CIs, \ie $\cup_{j \in J} \CI \subseteq \Sp$ for some $\CI \in \mathcal{S}^*_\alpha(e_j,\tilde{\tau}_j)$. Thus, we use the following conservative definition for CIs with multiple attack goals: $\Sp:= \cup_{j \in J} \CI$.  
\end{remark}
\vspace{-\dist}

